GeoFusion: Geometric Consistency informed Scene Estimation in Dense Clutter

We propose GeoFusion, a SLAM-based scene estimation method for building an object-level semantic map in dense clutter. In dense clutter, objects are often in close contact and severe occlusions, which brings more false detections and noisy pose estimates from existing perception methods. To solve these problems, our key insight is to consider geometric consistency at the object level within a general SLAM framework. The geometric consistency is defined in two parts: geometric consistency score and geometric relation. The geometric consistency score describes the compatibility between object geometry model and observation point cloud. Meanwhile, it provides a reliable measure to filter out false positives in data association. The geometric relation represents the relationship (e.g. contact) between geometric features (e.g. planes) among objects. The geometric relation makes the graph optimization for poses more robust and accurate. GeoFusion can robustly and efficiently infer the object labels, 6D object poses, and spatial relations from continuous noisy semantic measurements. We quantitatively evaluate our method using observations from a Fetch mobile manipulation robot. Our results demonstrate greater robustness against false estimates than frame-by-frame pose estimation from the state-of-the-art convolutional neural network.

==> GeoFusion 3/abstract.tex <==
\begin{abstract}
%For robots to perform useful tasks and interact fluently with human users, they must be able to 
We propose \textit{GeoFusion}, a SLAM-based scene estimation method for building an object-level semantic map in dense clutter.  In dense clutter, objects are often in close contact and severe occlusions, which brings more false detections and noisy pose estimates from existing perception methods. To solve these problems, our key insight is to consider geometric consistency at the object level within a general SLAM framework. The geometric consistency is defined in two parts: geometric consistency score and geometric relation. The geometric consistency score describes the compatibility between object geometry model and observation point cloud. Meanwhile, it provides a reliable measure to filter out false positives in data association. The geometric relation represents the relationship (e.g. contact) between geometric features (e.g. planes) among objects. The geometric relation makes the graph optimization for poses more robust and accurate. \GeoFusion  can robustly and efficiently infer the object labels, 6D object poses, and spatial relations from continuous noisy semantic measurements. We quantitatively evaluate our method using observations from a Fetch mobile manipulation robot.  Our results demonstrate greater robustness against false estimates than frame-by-frame pose estimation from the state-of-the-art convolutional neural network. %\cite{wang2019densefusion}. \chad{no citations in the abstract} %and outperforms the baseline methods that do not consider geometric consistency.
\end{abstract}

% continuously and  autonomously acquire information for decision making

% unstructured environment -> imperfectness of the world

%Our method enforces geometric consistency object geometries and the observed point cloud and the geometric relation between objects. The result provides a reliable measure to filter out false positives in data association, and more robust and accurate pose estimation through graph optimization.
%and poses geometric constraints in graph optimization for more robust and accurate pose optimization. 

==> GeoFusion 3/association.tex <==
\section{Data Association} \label{sec:da}

\begin{algorithm}[t]
\SetAlgoNoLine
\caption{Clustering Based Data Association}%
\label{alg:association}
\LinesNumbered 
\KwIn{Measurements $\mathcal{Z}$, Robot poses $\mathcal{X}$, Objects $\mathcal{O}$}
\KwOut{Data Associations $\mathcal{D}$}
\For {\textup{Each measurement $z_t^k$}}{
    \For{\textup{Each object $o_j$}}{
    \textup{Compute likelihood of $z_t^k$ of being object $o_j$:}\\
    $p(d_t^k=j) \propto  \mathbb I_{z^{k,c}_t =o_j^c} f_{gc}(z_t^k|o_j) f(z^{k, p}_t|o^{p}_j, x_t)$;\\
    }
    
    \eIf{$\max p_j \leq \epsilon_{new}$}
    {
        \textup{NewObjectInit($z_t^k$);}
    }
    {
        $d_t^k =\argmax p_j$;
    }
}

\For{\textup{Each object $o_j$}}{
    \textup{Compute false positive score} $f_j$ and remove it if score is above $\epsilon_{fp}$}

\end{algorithm}



% classify measurements, clusterstatesinit, measurementpreassociate, associate, 
% updateclusters, mergeclusters, updateobjects, removefalsepositive, removeobject, overlap, update measurements
%Even though the accuracy of object detection and 6D pose estimation has dramatically improved over the year, the correct association of measurements and objects based on their 6D poses remains a challenge, especially when they are in a cluttered environment.  
% That requires us to capture the false positives in the raw measurements at the same time. 

%As the robot moves in the world, multiple view measurements of the same scene are obtained from the state-of-the-art neural network object detector in consecutive frames. 
%We consider all the measurements from different frames together and proposed our clustering-based approach as shown in \ning{ref 2 alg}. In this algorithm, the key points are two-fold: One is to calculate the reliability score of each measurement by incorporating the corresponding depth and object geometry information, and adopt this attribute as a prior knowledge of each measurement in the following clustering operations. The other is to develop a thorough and robust process of removing false positives, even in a densely cluttered scene.     

% \ning{challenge and key points}



%Given initial estimates of objects $\mathcal{O}^{(0)}$, robot poses $\mathcal{X}^{(0)}$ and measurements $\mathcal{Z}$, 
As the number of objects $M$ is not known as the prior knowledge, we proposed a non-parametric clustering based approach for estimating data association in Eq. \ref{eq:da} based on DPmeans algorithm \cite{kulis2011revisiting}, as shown in Algorithm \ref{alg:association}.  Given initial estimates of objects $\mathcal{O}^{(0)}$, robot poses $\mathcal{X}^{(0)}$ and measurements $\mathcal{Z}$, we compute how likely each measurement belongs to current objects, being a new object or a false positive. The objects are created, updated, and deleted dynamically as the data association process moves forward. 


%For each measurement, we also consider the geometric consistency between measurements and raw point cloud by computing projective inlier, outlier and occlusion score for determining the quality of 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% The algorithm is shown as follows:


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \subsubsection{Geometric score}
% Before performing data association: 
% Describe how we select reliable measurements based on its pose rendering score. inlier, outlier, 
% This attribute of measurement can be considered as an initial evaluation of the reliability of each measurement. And this is the key attribute that we used to perform cluster merging(loop closure) and False Positive removal.\ning{Score Calculation Formula? }

%In our model, a cluster is denoted as $c_i$, where $c_i = \{c_i^p, c_i^c\}$, $c_i^p$ is the pose of i$th$ cluster in $SE(3)$ and $c_i^c$ is its class. A set of clusters $c_{1:N}$ are considered as object candidates in the semantic map. They are created, updated and deleted dynamically as the data association process moves forward. Moreover, several main attributes of each cluster, including 6D pose, class, reliability score $R_i$ and assigned measurements \{$z_t^k\}_i$ are also maintained through the process. 

% associate 公式 

% Starting from an empty map with unknown numbers and categories of objects, the measurements in every frame will be either assigned to an existed cluster or a new cluster when it doesn't meet the requirements of assigning to any existed cluster. Then a new cluster will be initialized with this measurement class and pose.




\subsubsection{Association}

%The association process is performed by classifying measurements into clusters based on their classes, reliability, and 6D pose similarity. It is worth noting that this process starts without any prior information on numbers or categories of objects in the scene at the very beginning. 

For each measurement $z^k_t$ in frame $t$, the likelihood of $z_t^k$ being assigned to object $o_j$ will be calculated as follows: 
\begin{equation}
    P(d_t^k=j) \propto  \mathbb I_{z^{k,c}_t =o_j^c} \, f_{gc}(z_t^k|o_j) \, f(z^k_t|o_j, x_t),
\end{equation}
where $\mathbb I_{z^{k,c}_t =c_i^c}$ is the label factor and it is obtained using an indicator function that evaluates to 1 if $z^{k,c}_t =c_i^c$ and 0 otherwise, meaning that each measurement will only be assigned to an object with the same label. %(Why)

%As mentioned before, $f_{gc}(z_t^k|c_i)$ represents one of the key attributes of each measurement and it serves as an initial evaluation of the measurement reliability. \ning{@sui Details and formula regarding this Geometry Score combination, geometric consistency} 



Second term $f_{gc}(z_t^k | o_j)$ captures the geometric consistency score between measurement and the observation point cloud and provides a measure of how reliable the given measurement is. The motivation behind this term is that the confidence score given by neural networks sometimes are not accurate enough to describe the reliability of the measurement. Given a measurement $z_t^k$, a point cloud is back-projected from the rendered depth image and compared with observation point cloud to compute projective inlier ratio $r_i$, outlier ratio $r_{out}$ and occlusion ratio $r_{occ}$. A point in the rendered point cloud is
first considered as an occlusion point if it is occluded by the projective point in the observation point cloud shooting from the camera ray. If not, it is considered as an inlier if the distance with the projective point is less than certain sensor resolution $\epsilon_{res}$, or outlier if the distance is greater than $\epsilon_{out}$. Fig. \ref{fig:inlier} shows an example of different types of points. The ratios are computed over the total number of rendered points. And they are used as follows:

\begin{equation}
    f_{gc}(z_t^k | o_j) = S(r_{i}) S(1 - r_{out})S(1 - r_{occ})
\end{equation}
where $S$ is a modified sigmoid function providing an S-shaped logistic curve that is well-adapted to reflect the changing tendency of confidence on the given measurement over different values of each ratio.

\begin{figure}[t]
    \centering
    %\includegraphics[width=0.48\textwidth]{images/measurements-000041.png}
   \includegraphics[width=0.9\textwidth]{images/inlier_score.jpg}
    \caption{\footnotesize Geometric consistency score between measurements and point cloud observation. The zoomed picture shows the inlier, outlier and occlusion points of a mustard bottle. Point cloud observations are shown in dark blue. Inlier points are shown in green, outlier in red and occlusion in orange.} %\sui{remove frame at the left image (too dark) and remove table cloud at right image}
    \label{fig:inlier}
\end{figure}

The last term $f(z^k_t|o_j, x_t)$ is the pose factor that reflects the similarity of measurement pose and object pose, given the current robot pose $x_t$. Here, we make the assumption that the likelihood of each measurement $z_t^k$ given the robot pose and the object pose follows a multivariate Gaussian distribution.
\begin{equation}
    f(z_t^k|o_j, x_t) \sim \mathcal{N}(x_t^{-1}\cdot o_j^p , Q)
\end{equation}
where $Q$ is the measurement noise matrix and this factor can thus be drawn from the Gaussian probability density function. 
With all the factors described above, $z_t^k$ is assigned to be the maximum likelihood object if the object is within a certain threshold $\epsilon_{new}$, otherwise, it is assigned to a new object.

% With all the factors described above, the assignment likelihood $P(d_t^k = i)$ is essentially proportional to the product of them. Each of the measurement will be assigned to the cluster with maximum likelihood if that likelihood exceeds $\epsilon$, the empirical constant of creating a new cluster. Otherwise, a new cluster will be created under the same class and pose as the measurement.

The One Measurement Per Object (OMPO) constraint \cite{wong2015data} is also applied in this process so that two measurements in the same frame will never be assigned to the same object and the latter will be assigned to a new object instead.
% It is beneficial to follow such a constraint as the potential false-positive measurements are supposed to be set apart instead of mixing them with reliable measurements in the same cluster.

% Moreover, the cluster reliability score \ning{cluster reliability score} 
\subsubsection{False positive removal}
%\begin{paragraph}{False positive score}
For each object candidate created or updated in the association step, we compute its false positive score $f_j$ as follows: 
\begin{equation}
f_j = 1 - \frac{R_j}{1+e^{(-n_j)}}  
\end{equation}
where $n_j$ is the number of measurements assigned to $o_j$ and $R_j$ is the maximum geometric consistency score among all of these measurements. 
If there are more measurements assigned to one object, it is reasonable to consider this object as more reliable among others thus it deserves a lower false-positive score. All objects with false-positive scores higher than $\epsilon_{fp}$ will then be deleted.
%  Therefore, the false positive likelihood $f_i$ is calculated for each cluster $c_i$ using the following equation, where $R_i$ is the cluster reliability score, $n_i$ is the number of measurements assigned to cluster $c_i$. All clusters that have a high false-positive likelihood will be filtered out and the rest portion will be associated with objects which inherit all the attributes from their corresponding clusters.

%\end{paragraph}


\begin{paragraph}{Overlapped objects merging}  % Why??
 We notice that most of the false positive measurements usually overlap with other objects, especially for symmetric objects, like a cylinder-shape tomato soup can. Object-level geometric consistency is incorporated again to address this problem as we applied Separating Axis Theorem (SAT) %\cite{gottschalk1996obbtree} 
 to detect the collision ratio of the three-dimensional bounding boxes of any two objects. Corner points of each bounding box are projected to several main axes and the overall collision ratio is decided based on the percentage of overlap along each axis. One object with a high collision ratio will be merged to the other one that has a lower false-positive score.% A Non-Maximum Suppression (NMS) algorithm \cite{neubeck2006efficient} is also adopted to ensure we find the best candidate when there are multiple objects that overlap with each other. 

 \end{paragraph}





==> GeoFusion 3/discussion.tex <==
\section{Conclusion}
In this work, we present \textit{GeoFusion}, a SLAM-based scene understanding method for building a semantic map at object-level in dense clutter while taking into account geometric consistency. Our method is able to infer object labels and 6D poses from noisy semantic measurements robustly and efficiently. The reasoning at object-level with geometry offers a fast and reliable way to filter out false positives and constraint the object through geometric relation. The computed geometric relations are also directly amenable to high-level task planners for robots to reason over actions for goal-directed manipulation tasks. %The results show that by considering geometric consistency our method is    

==> GeoFusion 3/experiments.tex <==
\section{Experiments}

\begin{table}
   % \normalsize
    \centering
    %\resizebox{\textwidth}{!}
    \begin{center}
% occlusion = 0.8
\begin{tabular}{ c|c|c|c|c } 
 \toprule
 & FbF & B-SLAM & R-Front & \GeoFusion  \\
 \midrule
$\text{mAP}_{50}$ & 58.4 & 56.0 & 72.3 & \textbf{73.4} \\ 
 \hline
$\text{mAP}_{75}$ & 28.6 & 24.6 & 50.3 & \textbf{59.5} \\ 
\hline
$\text{mAP}_{50:95}$ & 30.5 & 27.9 & 45.2 & \textbf{50.3} \\ 
 \hline
 
\end{tabular}
\end{center}
    \caption{\footnotesize Object detection performance of different methods with mAP under different IoU.  }
    \label{tab:object-detection}
\end{table}


\begin{table} % confidence score threshold: 0.5
    \footnotesize
    \centering
    %\resizebox{\textwidth}{!}
    \begin{center}
\begin{tabular}{c |cc|cc|cc|cc}
\toprule
  & \multicolumn{2}{c|}{FbF} & \multicolumn{2}{c|}{B-SLAM} & \multicolumn{2}{c|}{R-Front}  & \multicolumn{2}{c}{\GeoFusion} \\
   & Pr & Rec & Pr & Rec & Pr & Rec & Pr & Rec \\

%  \hline
%  & TP & FP & FN & TP & FP & FN & TP & FP \\
\midrule
 %\hline
 $\text{mAP}_{50}$ & 0.87 & \textbf{0.60} & 0.87 & 0.27 & 0.91 & 0.43 & \textbf{0.99} & 0.51 \\
 \hline
 $\text{mAP}_{75}$ & 0.56 & 0.38 & 0.63 & 0.19 & 0.75 & 0.35 & \textbf{0.91} & \textbf{0.46} \\
 \hline
 $\text{mAP}_{50:95}$ & 0.52 & 0.35 & 0.57 & 0.17 & 0.65 & 0.30 & \textbf{0.77} & \textbf{0.40} \\ 
 \hline
\end{tabular}
\end{center}
    \caption{\footnotesize Object detection performance on precision (Pr) and recall (Rec) for different methods under different mAP. The detection confidence threshold is set to 0.5. }
    \label{tab:object-detection-precision-recall}
\end{table}


% \begin{table}[]
%     \normalsize
%     \centering
%     %\resizebox{\textwidth}{!}
%     \begin{center}
% \begin{tabular}{ |c|c|c|c|c|c| } 
%  \hline
%  & TP & FP & FN & Precision & Recall \\
%  \hline
% \GeoFusion & 10.34 & \textbf{0.20} & 3.72 & \textbf{0.98} & 0.73 \\ 
%  \hline
%  FbF & 8.28 & 1.65 & 4.91 & 0.84 & 0.65 \\ 
%  \hline
% B-SLAM & 10.50 & 17.77 & 3.59 & 0.37 & 0.74 \\ 
%  \hline
% R-Front & \textbf{10.77} & 1.97 & \textbf{3.30} & 0.85 & \textbf{0.77}\\ 
%  \hline
% \end{tabular}
% \end{center}
%     \caption{Object detection performance on TP, FP and FN. TP, FP and FN refer to the true positives, false positives and false negatives averaged over each frame. }
%     \label{tab:object-detection-raw-numbers}
% \end{table}


% \begin{table}[] % confidence score threshold: 0.6
%     \footnotesize
%     \centering
%     %\resizebox{\textwidth}{!}
%     \begin{center}
% \begin{tabular}{c |cc|cc|cc|cc|}
% \toprule
%   & \multicolumn{2}{c|}{FbF} & \multicolumn{2}{c|}{B-SLAM} & \multicolumn{2}{c|}{R-Front}  & \multicolumn{2}{c|}{\GeoFusion} \\
%   & Pr & Rec & Pr & Rec & Pr & Rec & Pr & Rec \\

% %  \hline
% %  & TP & FP & FN & TP & FP & FN & TP & FP \\
% \midrule
%  %\hline
%  $mAP_{50}$ & 0.87 & 0.60 & 0.93 & 0.20 & 0.94 & 0.32 & 0.99 & 0.44 \\ 
%  \hline
%  $mAP_{75}$ & 0.56 & 0.38 & 0.72 & 0.15 & 0.31 & 0.80 & 0.91 & 0.40 \\ 
%  \hline
%  $mAP_{50:95}$ & 0.52 & 0.35 & 0.63 & 0.13 & 0.68 & 0.24 & 0.78 & 0.34 \\ 
%  \hline
% \end{tabular}
% \end{center}
%     \caption{Object detection performance on TP, FP and FN. TP, FP and FN refer to the true positives, false positives and false negatives averaged over each frame. }
%     \label{tab:object-detection-raw-numbers}
% \end{table}





\subsection{Implementation}
We use Mask R-CNN \cite{he2017mask} and DenseFusion \cite{wang2019densefusion} to generate semantic measurements where the former detects objects along with the instance segmentation which the latter takes in to estimate the 6D pose. We finetune the Mask R-CNN with the YCB-Video Dataset \cite{xiang2017posecnn} with the pretrained Microsoft coco model \cite{lin2014microsoft}. We use the public available DenseFusion weights and implementation without fine-tuning. The front-end in our implementation selects every 10th camera frame as a keyframe. The camera visual odometry is provided by ORB-SLAM2 \cite{murAcceptedTRO2015}. We use Ceres \cite{ceres-solver} as the optimization backend. In our implementation, we perform stage I optimization every 10th keyframe and perform stage II optimization every keyframe.

%data association \sui{@Ning: add parameters for data association} \\



\subsection{Dataset and Baseline}
To test the performance of our method, we collect a testing dataset \footnote{ \url{http://www-personal.umich.edu/~zsui/geofusion_dataset.html} } from six RGBD video streams in which our Michigan Progress Robot moves around the table. In each scene, we put around 18 objects in dense clutter on the table and collect around 200 keyframe RGB-D observations from the robot's sensor. %. \ref{fig:} shows the scene xx in the dataset. 
The groundtruth object classes and poses are labelled using LabelFusion \cite{marion2018label}. For baseline methods, we compare our method with frame-by-frame (FbF) estimation from Mask R-CNN and DenseFusion. It only considers the single frame and does not take any temporal or spatial constraints into account.  We also compare with the variations of our proposed \textit{GeoFusion}: 1) a baseline SLAM (B-SLAM) method without considering geometric consistency in both data association and graph optimization. The confidence score from DenseFusion instead of the geometric consistent score is used in computing data association. The back-end graph optimization only optimizes over odometry and object poses without considering spatial constraints between objects.  2) a robust front-end (R-Front) method where only our data association is used and not the graph optimization.





\begin{figure}[t]
    \centering
        \includegraphics[width=0.9\columnwidth]{images/pose_accuracy.eps}
       
    \caption{\footnotesize Pose accuracy comparison between different methods. }
    %\chad{it is not clear that Frame-by-Frame is DenseFusion}}
    \label{fig:pose_acc}
    \vspace{-2mm}
\end{figure}

\subsection{Evaluation} 
\subsubsection{Object Detection}
We first compare object detection performance with baseline methods on each keyframe collected in the dataset. 

\begin{paragraph}{mAP}
We use the common object detection metric: mean average precision (mAP), to evaluate object detection. Average precision (AP) is the area under the Precision-Recall curve of an object class and mean average precision is the mean of all the AP. The subscript under mAP is the ratio of intersection over union (IoU) between the estimated bounding box and the ground truth bounding box. %$\text{mAP}_{50}$ indicates a detection is a true positive if the IoU is over 0.5 and $\text{mAP}_{75}$ sets a more strict criteria where a detection is true positive only if the IoU is over 0.75. 
We also use mAP@[50:95] which corresponds to the average AP for IOU from 0.5 to 0.95 with a step size of 0.05.  

Results are shown in Table \ref{tab:object-detection}. \GeoFusion significantly outperforms the frame-by-frame method in all mAP metrics indicating that our method is capable of identifying false detections and keeping true ones from noisy semantic measurements. Robust front-end method achieves the similar $\text{mAP}_{50}$ with \GeoFusion however underperforms in $\text{mAP}_{75}$ and $\text{mAP}_{50:95}$. It shows that the back-end optimization improves the 6D poses of objects, which in turn increases the mAP with a tighter threshold in IOU. The baseline SLAM method does not take any geometric consistency into account and the performance is even worse than the frame-by-frame method. This is because the false and noisy measurements accumulate in the baseline slam and without the help of geometric consistency, they are difficult to be eliminated from the estimates. 
%there is no way to remove them  which in turn proves the geometric consistency play a vital role in semantic mapping at object-level. 
\end{paragraph}

\begin{paragraph}{Precision and Recall}
For a more intuitive evaluation on object detection, we also report numbers on precision (Pr) and recall (Rec) with the confidence score threshold set to 0.5. As shown in Table \ref{tab:object-detection-precision-recall}, \GeoFusion outperforms all the baseline methods under different mAP metrics. With the ratio of IOU increases for checking true positives, the performance gap between \GeoFusion and baseline methods becomes larger. Interesting, the recall of the Frame-by-frame method under $\text{mAP}_{50}$is higher than \textit{GeoFusion}. This is because \GeoFusion has a strict way to filter out false and noisy detections. In other words, detections are chosen very conservatively by \GeoFusion which leads to more false negatives in a looser metric. 
\end{paragraph}


%than baseline methods at precision and average false positives and comparable at recall showing that our method is capable of identifying false detections and keeping true ones. Robust front end method achieves the best true positives, false negatives and recall at the cost of increasing false positives which is caused by the drift with the unoptimized odometry.  Baseline SLAM has the similar true positives and false negatives however drastically high at false positives which in turn proves the geometric consistency play a vital role in semantic mapping at object-level.  


%The average true positives, false positives, false negatives, precision and recall ratio are computed. An detection is a true positive if the intersection over union (IoU) of its bounding box and the ground truth bounding box is over 0.5. The objects in severe occlusions are not counted. 
% Note that our method requires some time to accumulate measurements to build the semantic map and for fair comparison with frame-by-frame method, the first few frames are still included in the evaluation. 
%Results are shown in Table \ref{tab:object-detection}. Our method significantly outperforms than baseline methods at precision and average false positives and comparable at recall showing that our method is capable of identifying false detections and keeping true ones. Robust front end method achieves the best true positives, false negatives and recall at the cost of increasing false positives which is caused by the drift with the unoptimized odometry.  Baseline SLAM has the similar true positives and false negatives however drastically high at false positives which in turn proves the geometric consistency play a vital role in semantic mapping at object-level.  



\subsubsection{Pose Accuracy} For 6D object pose accuracy, we use the ADD-S metric \cite{xiang2017posecnn} to compute the average point distance between estimated pose and the correct pose. Only true positives are computed at each frame for each method. As our aim is to build a high accuracy object-level map and the precision required by the robot to grasp objects are relatively high, we plot the accuracy-threshold curves within the range of [0.00m, 0.02m] as shown in Fig. \ref{fig:pose_acc}. \GeoFusion achieves the highest pose accuracy among all the methods and about 90\% percent of the objects have achieved pose error under 1cm. The pose accuracy of baseline SLAM method is even worse than the Frame-by-Frame method indicating that the confidence scores from perception module are sometimes not reliable. 
%\subsubsection{Geometric Relation} Fig. \ref{fig:geometry_relation_compare} in Appendix shows the comparison of two stage optimization 
%\subsubsection{Run Time}
%Except from the measurements generation, our method (data association and graph optimization) only runs on CPU and the average time for each frame is under 200ms. 


%We show an run time analysis on each frame for data association and optimization of an example scene in Fig. \ref{fig:teaser}. Note that our method only runs on CPU (without measurements generation), the average time for each frame is under 200 ms

% We show an run time analysis on each frame for data association and optimization of an example scene in Fig. \ref{fig:teaser}. Note that our method only runs on CPU (without measurements generation), the average time for each frame is under 200 ms. 
% \begin{figure}[t]
%     \centering
%         \includegraphics[width=0.9\columnwidth]{images/time_plot.eps}
%     \caption{\footnotesize Time plot for each frame of the scene in the Fig. \ref{fig:teaser}} 
%     \label{fig:time_plot}
% \end{figure}


\subsubsection{Run Time}
% Except from the measurements generation, our method (data association and graph optimization) only runs on CPU and the average time for each frame is under 200ms. 

We show an analysis of run time in Fig. \ref{fig:time_plot} on each frame for data association and optimization of an example scene in Fig. \ref{fig:teaser}. Note that our method only runs on CPU (without measurements generation), the average time for each frame is under 200 ms

%We show an run time analysis on each frame for data association and optimization of an example scene in Fig. \ref{fig:teaser}. Note that our method only runs on CPU (without measurements generation), the average time for each frame is under 200 ms. 

\subsubsection{Geometric Relation} Fig. \ref{fig:geometry_relation_compare} compares the results of two optimization stage of the scene in Fig. \ref{fig:teaser}. Left figure is the result of optimization stage I without geometric relation constraints and the right figure is the result after optimized over geometric constraints. The geometric constraints pulled objects to satisfy the constraints. For example, the objects on the right are more aligned with the table and the intersection between objects is fixed. 

\begin{figure}[t]
    \centering
        \includegraphics[width=0.9\columnwidth]{images/time_plot.eps}
    \caption{\footnotesize Time plot for each frame of the scene in the Fig. \ref{fig:teaser}} 
    \label{fig:time_plot}
\end{figure}

\begin{figure*}[]
    \centering
        \includegraphics[width=0.45\columnwidth]{images/wo_geometry_white_bg.png}
        \includegraphics[width=0.45\columnwidth]{images/w_geometry_white_bg.png}
    \caption{\footnotesize The comparison of the two-stage optimization of 230th keyframe of the scene in Fig. \ref{fig:teaser}.% The left figure shows the result after stage I optimization and the right figure shows the result after stage II optimization with geometric relation constraints. It's clear that the geometric constraints pull each object satisfying the constraints and make the entire scene more geometrically stable.
    } 
    \label{fig:geometry_relation_compare}
\end{figure*}

==> GeoFusion 3/formulation.tex <==
\section{Problem Formulation}
Our aim is to estimate the semantic map composed of a collection $\mathcal{O} = \{ o_j \}_{j=1}^M$ of $M$ static objects as well as geometric relationships $\mathcal{R} = \{r_{ij} | i, j \in [1, M] \}$ between them with the assumption of known 3D object geometries. Note that the number of objects $M$ is unknown. Each object $o_j = (o_j^c, o_j^p)$ contains object class $o_j^c \in [1, C]$ and 6D object pose $o_j^p \in SE(3)$. Each $r_{ij}$ describes the geometric spatial relation between geometric features of two objects (e.g. support), more of which will be discussed at Sec. \ref{sec:geometric_relations}.

When the robot moves around in the environment, it observes a set of semantic measurements %$\mathcal{Z} = \{ \{z_t^k\}_{k=1}^{N_t} , I_t\}_{t=1}^T$, 
 $\mathcal{Z} = \{ \{z_t^k\}_{k=1}^{N_t}\}_{t=1}^T$, 
where $T$ is the total time step robot has travelled, %$I_t$ is the point cloud observed at time $t$  
and $N_t$  is the number of semantic measurements at each time step. Similar to the definition of object, each semantic measurement $z_t^k = (z_t^{k,c}, z_t^{k,p})$ is comprised of object class and 6D pose. The robot poses represent as $\mathcal{X} = \{x_t\}_{t=1}^T$, where $x_t \in SE(3)$ is also 6D pose in our case. In addition, the correspondence between objects $\mathcal{O}$ and measurements $\mathcal{Z}$ also needs to be determined and is defined as $\mathcal{D} = \{ \{d_t^k\}_{k=1}^{N_t} \}_{t=1}^T $ where $d_t^k = j$ stipulates that measurement $z_t^k$ corresponds to object $o_j$.

A complete statement of this problem is the maximum likelihood estimation of $\mathcal{X}$, $\mathcal{O}$, and $\mathcal{D}$ given the semantic measurements $\mathcal{Z}$ and the geometric relation $\mathcal{R}$ is computed heuristically from $\mathcal{O}$:

\begin{equation} \label{eq:overall-optimization}
    {\hat{\mathcal{X}}}, {\hat{\mathcal{O}}},  {\hat{\mathcal{D}}} = \argmax_{\mathcal{X}, \mathcal{O},  \mathcal{D}} \log p(\mathcal{Z} | \mathcal{X}, \mathcal{O},  \mathcal{D})
\end{equation}

As the joint estimation of objects, data association and robot poses suffers from the high dimensionality, 
the most common approach is to decompose Eq. \ref{eq:overall-optimization} into two separate estimation problems: data association and graph optimization.
%we decompose it into two separate estimation problems. \newtext{The decomposition follows the standard SLAM framework. Some early work should be cited }
The maximum likely estimation data association $\mathcal{D}$ is first computed given initial estimates of robot poses $\mathcal{X}^{(0)}$ and objects $\mathcal{O}^{(0)}$. Then given computed $\hat{\mathcal{D}}$, the most likely robot poses and objects are estimated:

\begin{align} 
    \hat{\mathcal{D}} &= \argmax_{\mathcal{D}}  p(\mathcal{D} | \mathcal{X}^{(0)}, \mathcal{O}^{(0)}, \mathcal{Z})  \label{eq:da} \\
       {\hat{\mathcal{X}}}, {\hat{\mathcal{O}}}  &= \argmax_{\mathcal{X}, \mathcal{O}} \log p(\mathcal{Z} | \mathcal{X}, \mathcal{O},  \hat{\mathcal{D}}) \label{eq:optimization}
\end{align}

Again, we decompose Eq. \ref{eq:optimization} to a two-step optimization where the object and robot poses are first optimized and the geometric relation $R$ will be computed heuristically from $O$ and these geometric relations will, in turn, pose constraints on factor graph for estimating geometrically stable scene: %motivation for decomposing the optimization into two steps
\begin{align} 
       {\hat{\mathcal{X}}}, {\hat{\mathcal{O}}}^{'} &= \argmax_{\mathcal{X}, \mathcal{O}} \log p(\mathcal{Z} | \mathcal{X}, \mathcal{O},  \hat{\mathcal{D}}) \label{eq:optimization-stage1} \\
       {\hat{\mathcal{O}}} &= \argmax_{\mathcal{O}} \log p(\mathcal{Z} | \mathcal{O}, \mathcal{R}) \label{eq:optimization-stage2} 
\end{align} 

%  In the following sections, we will describe how geometric consistency can be explored in data association in Section \ref{sec:da} and graph optimization over poses in Section \ref{sec:optimization} respectively. 

==> GeoFusion 3/geometry_constraints.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth] {images/surface_feature.png}
    \caption{\footnotesize Two types of surface feature: the left one is plane surface feature, and the right one is curved surface feature.}
    \label{surface feature}
\end{figure}
\subsection{Object Geometric Relationship Inference} \label{sec:geometric_relations}
%In Eq. \ref{eq:stage1-least-square}, 
In stage I optimization, the maximum likelihood estimation of robot and object poses is obtained by minimizing the odometry and object measurement cost. However, the resulting object poses are still noisy and not accurate enough for applications like precise robot manipulation. The noisy object poses lead to geometrically inconsistent scene estimate, e.g., floating or intersection between objects. To get a highly accurate and geometrically consistent scene estimate, we posit that if the geometric relationship between objects can be inferred and these relations can serve as the constraints (factors) between objects in the factor graph model, as shown in the right of Fig. \ref{factor graph}. Given estimated object poses $\mathcal{O}$ from Eq. \ref{eq:stage1-least-square}, $\mathcal{R}$ is heuristically computed.  

\subsubsection{Geometric Surface Feature} 
For common rigid household objects, we only consider \textit{contact} relations between surfaces for generality in representing the geometry of the object and efficiency in the graph optimization process. In this paper, geometric surface features are divided into two classes: plane surface feature and curved surface feature. An illustration of surface features is shown in Fig \ref{surface feature}.

Given an arbitrary convex polyhedron, geometric surface features can be extracted. For example, there are six plane surfaces and twelve curved surfaces for a cube-like geometry as it has six planes and twelve edges. The edge is treated as a zero radius curve surface. For cylinder-like geometry, there are two plane surfaces and one curved surface. Although the two classes of surfaces cannot represent all of the objects (e.g., articulated or non-rigid objects), they are general and sufficient for common rigid household objects.





%In real world, geometric relationship between objects can be really complicated. One object can support the other one, be parallel to the other one, or be perpendicular to the other one.
%If we want to use geometric relationship to optimize object poses, we have to be really conservative to those relationship. A wrong inference will be disastrous to the entire optimization.  

%For this reason, contact relationship is the only geometric relationship we choose for optimization. As we believe contact relationship is the most common and reliable geometric relationship between objects in real scenes, for objects in real scenes have to be put on something and contact with other objects.

%\newtext{talk about motivations of contact relationships used in this work}

%\subsubsection{Geometric Surface Feature}
%Surface geometric features are the keys to determine the existence of contact between different objects. In order to model the  geometry of object as general as we can, instead of modeling a object as a particular 3D shape like cube, cylinder and etc, a bunches of surface features are used to represent 3D geometry of an object. Through this way, an arbitrary convex polyhedron can be easily handled since it can be represented by a set of plane surface features. 

%In this paper, geometric surface features are divided into two classes: plane surface feature and curved surface feature. An illustration of those surface features is shown in Fig \ref{surface feature}.


\begin{paragraph}{Plane Surface Feature}
The plane surface feature refers to those planes on polyhedrons. There are three attributes associated with plane surface feature: a center point $C_p \in R^3$, a set of points $B_p = \{b^i_p\}_{i=1}^{N_b}$ with $b^i_p \in R^3$, and the normal direction $N_p \in R^3$. $C_p$ describes the 3D position of the plane center. Each $b^i_p$ is the 3D position of a boundary point on the surface and $N_b$ is the number of boundary points.  

%which describes the 3D position of the plane center, a set of points $B_p = \{b^i_p\}_{i=1}^N_b$ w Each $b_p^i$ is the 3D position of a boundary point of the surface and $M$ is the total number of boundary points. Normal direction $N_p \in R^3$, is the normal direction of plane feature in object local frame.
\end{paragraph}

\begin{paragraph}{Curved Surface Feature}
The curved surface feature describes curved surfaces in 3D shapes like cylinders. Noticeably, edges of polyhedrons are also regarded as a curved surface feature with a radius equal to zero. Five attributes are associated with the curved surface feature: $C_c \in R^3$ and $N_c \in R^3$, determining the 3D position of center and direction of the rotation axis of the curved surface. $B_c = \{b_c^i\}_{i=1}^2$ with $b_c^i \in R^3$ refers to the 3D position of boundary points in rotation axis. Radius $r$ describes the radius of the curved surface.
\end{paragraph}

Accordingly, we define three types of spatial relations between these two surfaces: Plane2Plane Contact (P2P), Plane2Curve Contact (P2C), and Curve2Curve Contact (C2C). Fig \ref{geometric relationship} illustrates these geometric relations.


%Based on above surface features, we can get three different types of contact relationship between features. They are plane-plane contact (P2P), plane-curved surface contact (P2C), curved surface-curved surface(C2C) contact. Fig \ref{geometric relationship} illustrates these geometric relations graphically. 

\subsubsection{Geometric Feature Relationship Inference}
\begin{paragraph}{P2P contact}
If two different plane surface features $P_u,\ P_v$ from two objects $o_i,\ o_j$ are contacting each other, their attributes should follow the following rules:
\begin{equation}
\begin{array}{c}
|T_{o_i}N_{P_u}^i \cdot T_{o_j}N_{P_v}^j + 1| < \epsilon_n^{pp} \\
|T_{o_i}N_{P_u}^i \cdot (T_{o_j}C_{P_v}^j - T_{o_i}C_{P_u}^i)| < \epsilon_c^{pp} 
\end{array}
\end{equation}
where $\epsilon_n^{pp}, \epsilon_c^{pp}$ are the direction threshold and distance threshold for P2P contact. %explain two equations here
\end{paragraph}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.8\linewidth] {images/geometric_relationship.png}
    \caption{\footnotesize Illustrations for geometric relationships. Plane to plane (P2P) contact, plane to curved surface (P2C) contact, and curved to curved surface (C2C) contact are shown from the left to the right. }
    \label{geometric relationship}
    \vspace{-2mm}
\end{figure*}

\begin{paragraph}{P2C contact}
If a plane surface feature $P_u$ and a curved surface feature $C_v$ are contacting each other, their attributes should follow the following rules:
\begin{equation}
\begin{array}{c}
|T_{o_i}N_{P_u}^i \cdot  T_{o_j}N_{C_v}^j| < \epsilon_n^{pc} \\
|T_{o_i}N_{P_u}^i \cdot (T_{o_j}C_{C_v}^j - T_{o_i}C_{P_u}^i) - r_j| < \epsilon_c^{pc}
\end{array}
\end{equation}
where $\epsilon_n^{pc}, \epsilon_c^{pc}$ are the direction threshold and distance threshold for P2C contact.
\end{paragraph}

\begin{paragraph}{C2C contact}
If two different curved surface features $C_u,\ C_v$ are contacting each other, their attributes should follow the following rules:
\begin{equation}
   |(T_{o_i}N_{C_u}^i \times T_{o_j}N_{C_v}^j) \cdot (T_{o_j}C_{C_v}^j - T_{o_i}C_{C_u}^i) - (r_i + r_j)| < \epsilon_c^{cc}
\end{equation}
where $\epsilon_c^{cc}$ is the distance threshold for C2C contact. 
\end{paragraph}

%More illustrations about those contact relationship can be found in Fig \ref{geometric relationship} in Appendix \ref{appendixA}.
% \subsubsection{Physical Relationship Check}
% Apart from using geometric methods to determine the contact relationship between objects, physical based checking are also used in geometric relationship inference. More details can be checked in Appendix \ref{appendixA}.


\subsubsection{Physical Relationship Check}
We also add two physical based check in complement to the above geometric methods to ensure eliminating false detected contact. For example, if two cubes are placed parallel and close to each other on the table, a P2P contact can be detected. However, there is a chance that those objects are just near to each other but not contacting each other. 


%Apart from using geometric methods to determine the contact relationship between objects, physical based checking are also used in geometric relationship inference. 


%By using geometric based method, we can find many contact feature pair candidates in a scene. However, not all candidates can be used in optimizations. Because there are still many false contact inference in this way. For example, if two cubes are placed parallel and close to each other on the table, we can detect a P2P contact between these two objects. But there is a chance that those objects are just near to each other but not contacting each other. To avoid those false contact judgment, we add two more physical checks for those contact feature pair candidates. The main idea is that we only consider those contact relationship resulted from gravity, which in other word, those support relationship.

\begin{paragraph}{Support direction check}
If a plane feature can support another plane or be supported, its normal direction can not be horizontal to the gravity direction. Assume the direction of gravity is $N_G$, the support direction check of plane feature $i$ is defined as:
\begin{equation}
    N_G \cdot N_p^i > \epsilon_G
\end{equation}
where $\epsilon_G$ is the threshold for support direction check.
\end{paragraph}
Here we make an implicit assumption that there is at least one grounded object, e.g. table, which supports all the other objects. Similar assumption can be found in SLAM++ \cite{salas2013slam++}.

\begin{paragraph}{Qualitative Support projection check}
If there is a support relationship between two features, their 2D projections along the direction of gravity must be overlapped. For those contact feature candidates, their 2D projections are the polygon or the edge projected from their boundary points. Separate axis theorem (SAT) is applied to check the overlapping of those 2D contours. Those feature candidates whose 2D projections are not overlapped will be removed.
\end{paragraph}

\subsection{Stage II Optimization}
After spatial relations $\mathcal{R}$ between objects have been computed from the estimated object poses in stage I optimization, these relations are used as constraints in the factor graph optimization. These constraints will enforce proper contact between objects and fix the issues of floating and interpenetration. We can rewrite the right hand side of Eq. \ref{eq:optimization-stage2} as:

\begin{equation}
     \log p(\mathcal{Z} | \mathcal{O}, \mathcal{R}) = \sum_{i=1}^M \sum_{j=1}^M \phi (r_{ij} ; o_i^p, o_j^p) \sum_{i=1}^M \phi(o_i^{'} ; o_i)
\end{equation}
where $\phi (r_{ij} ; o_i^p, o_j^p)$ is the geometric relation factor and $\phi(o_i^{'} ; o_i)$ is the object prior factor. The object prior factor comes from the estimated object poses in stage I optimization. The geometric relation factor encodes the contact constraint between two objects computed from the previous section. Accordingly, there are three constraints: P2P, P2C, and C2C. For P2P constraint, the cost function is defined as: 
\begin{equation}
    E_{P2P} =  \omega_q |T_{o_i}N_{P_u}^i \cdot T_{o_j}N_{P_v}^j + 1|  +  \omega_p
|T_{o_i}N_{P_u}^i \cdot (T_{o_j}C_{P_v}^j - T_{o_i}C_{P_u}^i)| \nonumber
\end{equation}
Similarly, the cost function of P2C constraint is defined as:
\begin{equation}
    E_{P2C} =  \omega_q | T_{o_i}N_u^{o_i} \cdot T_{o_j}N_v^{o_j} | 
    + \omega_p |T_{o_i}N_u^{o_i} \cdot (T_{o_i}C_u^{o_i} - T_{o_j}C_v^{o_j})| \nonumber
\end{equation}
and the cost function of C2C is defined as:
\begin{equation}
    E_{p2c} = \omega_p |(T_{o_i}N_u^{o_i} \times T_{o_j}N_v^{o_j}) \cdot (T_{o_i}C_u^{o_i} - T_{o_j}C_v^{o_j}) 
    - (r_v + r_u)| \nonumber
\end{equation}

%Geometric constraints between two objects are the combination of geometric constraints between their features, in another word, those P2P, P2C and C2C relationship. 

% \begin{paragraph}{P2P constraints}
% Given two objects, $o_i$ and $o_j$. If a P2P contact is detected between their plane feature $P_u,\ P_v$. Denote the relative transform of those features to the corresponding objects as $T^{o_i}_{P_u}, T^{o_j}_{P_v}$. (The local coordinate of a feature is a coordinate whose origin is located at $C_p$ and z-axis is equal to $N_p$.)

% Then we can make optimization over $o_i$ and $o_j$ to minimize the following cost:
% \begin{equation}
% \begin{array}{rl}
%   E_{P2P} =  \omega_q |T_{o_i}N_{P_u}^i \cdot T_{o_j}N_{P_v}^j + 1| \\ +  \omega_p
% |T_{o_i}N_{P_u}^i \cdot (T_{o_j}C_{P_v}^j - T_{o_i}C_{P_u}^i)| \\

    


%   T^u_v &= (T_{o_i}T_{P_u}^{o_i})^{-1} (T_{o_j}T_{P_v}^{o_j})\\
%   (q^u_v, p^u_v) & = F(T^u_v)\\
%   E_{P2P} &= ||q^u_v||_{\Sigma_q}+ ||p^u_v||_{\Sigma_p}
% \end{array}
% \end{equation}
% \begin{equation*}
%  \Sigma_p = Diag(0, 0, \omega_p),\ 
% \Sigma_q = Diag(0, \omega_q, \omega_q, 0)
% \end{equation*}
% %where the $\omega_p$ is the weight of distance constraints for P2P constraints, and $\omega_q$ is the weight of rotation constraints for P2P constraints.
% \end{paragraph}

% \begin{paragraph}{P2C constraints}
% Given two objects, $o_i$ and $o_j$. If a P2C contact is detected between their plane feature $P_u$ and curved surface feature $C_v$. We make optimization over $o_i$ and $o_j$ to minimize the following cost:
% \begin{equation}
% \begin{array}{rl}
%   E_{P2C} = & \omega_q | T_{o_i}N_u^{o_i} \cdot T_{o_j}N_v^{o_j} | \\
%   & + \omega_p |T_{o_i}N_u^{o_i} \cdot (T_{o_i}C_u^{o_i} - T_{o_j}C_v^{o_j})|
% \end{array}
% \end{equation}
% %where the $\omega_p$ is the weight of distance constraints for P2C constraints, and $\omega_q$ is the weight of rotation constraints for P2C constraints.
% \end{paragraph}

% \begin{paragraph}{C2C constraints}
% Given two objects, $o_i$ and $o_j$. If a C2C contact is detected between their curved surface features $C_u$ and $C_v$. we can optimize over $o_i$ and $o_j$ to minimize the following $C2C$ cost.
% \begin{equation}
% \begin{array}{rl}
%   E_{p2c} =& \omega_p |(T_{o_i}N_u^{o_i} \times T_{o_j}N_v^{o_j}) \cdot (T_{o_i}C_u^{o_i} - T_{o_j}C_v^{o_j}) \\
%   & - (r_v + r_u)|
% \end{array}
% \end{equation}
% %where the $\omega_p$ is the weight of distance constraints for C2C constraints.
% \end{paragraph}

==> GeoFusion 3/implementation.tex <==
\section{implementation}
\subsection{Object Detection and Pose Estimation}

For particle filtering, we employ the CUDA-OpenGL
interoperation to render all particles in a single render buffer
on the GPU and can be accessed by the CUDA kernels to
compute the weights for particles. The major computation
is operated on directly on GPU and there is very few data
transfer between GPU and CPU memory. It provides a
tractable solution for us to employ more particles to sample
hypothesized objects
\subsection{Grasp and Place}
Graspable poses for each objects are generated based on geometry models or using grasp points generator(GPG) in local frame. A point cloud based collision checker is implemented. All collision free graspable poses are kept and ranked. Graspable poses whose grasp points are closer to the center of target objects and whose axes through both finger tips are more parallel to the surface of table (to avoid poses where one finger is under objects) are given higher priority. 

Objects are placed according to a placing policy. In the placement algorithm, all the objects are represented by cuboids, and will be placed firmly on a plane. We use RANSAC to segment horizontal planes from the point cloud of the box and search among the planes to find a rectangle area with enough support for objects (either the center of the objects should be projected in the polygon surrounded by the support points or more than 70\% area around the center are supported). Place poses are ranked according the closeness to the ideal placement height given by the planner. Among the place poses with similar height, a better place position for regular object is close to the back center of the box; for vertical objects, a better pose is close to the two sides of the box. After checking the collision between the poses of objects and gripper with box point cloud, the place poses are given to MoveIt! to perform motion planning afterwards.

==> GeoFusion 3/introduction.tex <==
\section{introduction}
% What is your problem?

\IEEEPARstart{T}{o} make autonomous robots taskable such that they function properly, meet human expectations, and interact fluently with human partners, they must be able to perceive and understand the semantics of their environments~\cite{laird2017interactive}. More specifically, as robots move around in the environment, they must know what objects are presented as well as their locations. It is desired for robots to understand the semantic aspects of the scene and build a map at the object-level. %For example, our robot builds a semantic map around objects in Fig. \ref{fig:teaser} so it can perform meaningful tasks like grocery packing.  
An object-oriented representation of the world is a natural and efficient way for robots to make high-level decisions using task-level planners and help them to communicate with human users. 
%\ning{Define semantic map?}

%For robots to perform high-level tasks like objects searching or packing groceries, they must be able to identify semantic and task-relevant information (e.g. object identity and pose) in the environments and reason over actions towards satisfying goals. These actions are commonly generated by task-level planners, which in turn require an object-level representation of the world. Thus, it is desired for the robot to create a semantic world model of their surroundings that are structured around objects, their poses and spatial relations between them. Fortunately, techniques for object detection and 6D pose estimation have been greatly improved with the renaissance in deep neural networks \cite{ren2015faster, liu2016ssd, he2017mask, xiang2017posecnn, wang2019densefusion}, which greatly benefit the construction of the semantic world model. However, detections and estimations from these neural networks are sometimes very noisy due to the bias and lack of diversity in the training dataset, especially in the complex real environments the robots are facing. On the other hand, these single-view perception methods are insufficient in densely cluttered scenes where there is partial or complete occlusion among objects and large viewpoint variations. In this paper, we aim to build a robust object-level semantic model from continuous noisy observations provided by perception modules in cluttered scenes. 


% What are the challenges?

The challenge is that many semantic aspects of the world are difficult for robots to sense directly due to the limited field-of-view and noisy observations from their onboard sensors.  Great progress has been achieved by the advances in deep neural networks for object detection \cite{ren2015faster, liu2016ssd, he2017mask} and 6D object pose estimation \cite{xiang2017posecnn, tremblay2018deep, wang2019densefusion}. % and semantic segmentation \cite{long2015fully, papandreou2015weakly}.
However, building a semantic map at the object-level remains a challenging problem, especially in densely cluttered environments such as the one shown in Fig. \ref{fig:teaser}. Because in such dense clutter, objects are often in close contact, causing severe or complete occlusions.

% Objects in dense clutter are often in close contact 

%These advances depend on sufficient training data and well-designed models and the detections are often times noisy in unforeseen environments due to the complex and dynamic nature of the real world. The performance becomes worse in densely cluttered environments as shown in Fig. \ref{fig:teaser} where there are partial or complete occlusion among objects and multiple objects are in close contact.  


% Promising Approach
One promising approach for building object-level maps is to fuse semantic measurements from different viewpoints. Robots can take advantage of their ability to move around the environment and provide continuous observations. %\chad{I do not understand the next sentence:} 
More specifically, the data association between measurements and objects are first determined~\cite{wong2015data} and probabilistic model are built over objects and robot poses to infer the semantic map (SLAM++ \cite{salas2013slam++}, Fusion++ \cite{mccormac2018fusion++}) or belief over objects (CT-MAP \cite{zeng2018semantic}). Such methods perform inference directly on the object instance instead of low-level primitives (points, surfels).  This approach to inference offers faster inference, more compact map representation, and the potential for dynamic object reasoning. We posit that %better words?? 
this approach is particularly advantageous %for constructing semantic map 
in dense clutter. The geometric properties of object instances and geometric relationships between objects can be used for more robust data association and accurate pose estimation.

%measurements from percetion modules 


%One solution to this problem is to perform 3D dense reconstruction \cite{newcombe2011kinectfusion, whelan2015elasticfusion} which fuses 3D point clouds at the geometric level from consecutive views first, and then segment and identify objects from the fused point cloud \cite{tateno20162, li2016incremental}. These methods work well in large scale environments however becomes fragile when the scene becomes densely cluttered where multiple objects are placed in close contact or there are substantial false positive observations. Another way is to directly perform fusion on higher level semantics like object identities and 6D poses and optimize over object pose graph \cite{salas2013slam++, mccormac2018fusion++}. We more interested in this direction since an awareness of object instance as the observations can provide more meaningful information when facing more cluttered scenes as shown in Fix xx. 



In this work, we present \textit{GeoFusion}, a SLAM-based approach for inferring object labels and 6D poses from continuous noisy measurements in dense clutter by exploring the \textit{geometric consistency} of the object instances. %\sui{definition of geometric consistency} %\ning{Here we define the geometric consistency as the consistency between objects and measurements or differenet objects under the same scene, with respect to point matching, pose similarity and spatial relation rationality. The benefit of introducing geometric consistency is twofold. First, it adds more constraints for an optimization problem over object poses, towards a more robust and accurate pose estimation. Second, the object spatial relations could also enable the robot to make better decisions regarding motion planning, objects manipulation or other high-level tasks.} 
 The geometric consistency is defined in two parts: geometric consistency score and geometric relation. The geometric consistency score describes the compatibility between the object geometry model and the observation point cloud. Meanwhile, it provides a reliable measure to filter out false positives in data association. The geometric relation represents the relationship (e.g. contact) between geometric features (e.g. planes) among objects. Moreover, geometric relation is directly amenable to make better decisions for high-level task planners. %\cite{PDDL:1998, asp}. 

Given noisy measurements from state-of-the-art object detection \cite{he2017mask} and pose estimation \cite{wang2019densefusion} systems, our method first determines the correct correspondences between measurements and objects with geometric consistency between measurements and point cloud observations. The associations are then used to build a factor graph along with the geometric relations between objects. We use the fast optimization technique to get the maximum likelihood estimation of object and robot poses. We quantitatively evaluate our method and demonstrate that \GeoFusion is able to estimate geometrically stable scene and be robust against false estimates from state-of-art frame-by-frame estimation system \cite{wang2019densefusion} and outperforms the baseline methods that do not consider geometric consistency.

%examined the geometric consistency between measurements and raw point cloud observations in eliminating false measurements and determining the correct correspondences between measurements and objects. After the objects are determined in the data association, the geometric consistency between objects are explored to provide geometric level spatial relations (e.g. plane to plane support) for better optimization over object poses. These object to measurements and object to object geometric consistency are modelled as in factor graph along with the constraints between robot poses. \sui{benefit of geometric relation} \ning{Some descriptions in this paragraph are redundant now}We quantitatively evaluate our method in densely cluttered scenes and show that our method produces robust and accurate result compared to state of art per-frame estimations.

%In this work, our goal is to estimate the semantic map consisting of object classes and 6 degree-of-freedom poses from the densely cluttered environment as shown in Fig xx, given noisy observations from perception modules. We propose a robust slam-based approach to construct an object-level map while considering the geometric consistency between measurements and 3D point clouds and spatial relations between objects. The geometric consistency captures how consistent the measurement given by neural networks with the raw 3D points and is used in data association stage to filter out false positives. We also explore the spatial relationship between objects to optimize the object poses. %We quantitatively evaluate our approach in terms of object detection and pose estimation accuracy and show that our approach 



% Due to noise, occlusion, and sensors’ limited field of view, observations


% Major challenges in single-view perception are partial or complete occlusion among object instances, large viewpoint variations of the same object class, and similar appearances shared across different semantic categories. These often occur in densely cluttered scenes, where multiple objects are in close contact and placed over a complex background

% These are rather qualitative single 3D snapshots rather than the more precise mapping we need for a robot to navigate.


% are often times noisy in the wild, due to biases and insufficient diversity in training dataset. 

%In our work, we aim to be robust to false detections from such networks. We model the object class as part of our hidden state for generative inference, rather than making hard decisions on class labels as given by the detector. Given

% First paragraph
% - For robots to operate in unstructured environments, they need to be able to sense-plan-act. 
% task-relavant information. for example, objects searching and packing groceies objects 
% it is appropriate for robots to construct ‘‘mental models’’ of their environment that are structured around objects, their properties, and their rela- tions to one another.  
% - Neural networks good and bad  cite to (posecnn, densefusion, maskrcnn)
% - rather than single view, we would like to incorprate continouos observations
% - our goal is to build an object-level semantic world from noisy conitnous obervations exploring geometric and context consistency between observations and objects. 

% Second paragraph
% - Existing approaches to semantic world modeling 
% -- fuse low-level features and do pose estimation on fused segmentation
% --- midfusion (heavy clutter)
% -- fuse object poses 
% --- data association from partial view (odometry)
% --- slam++ (large scale, large object non clutter) (object indepedent)

% % -- filtering-based approach
% % --- ct-map, sum (odometry? expensive computation)

% Third paragraph
% - Our approach and contribution
% -- robust data associaiton
% -- factor graph optimization with context spatial relationship between objects


% Structure of the paper



%To achieve robust, autonomous operation in unstructured
% environments, robots must be able to identify relevant objects and features in their surroundings, recognize the context of the situation, and plan their motions and interactions accord- ingly.

%Scene understanding is a key enabling component for intelligent systems that can interact with human and physical environments. Over the past few years, substantial progress has been made by deep learning methods for single-view object classification [1], [2], [3], [4], [5], semantic seg- mentation [6], [5], [7], [4], and object pose estimation [8]. However, none of these recognition systems achieve suffi- ciently fast and accurate perception performance as required by most robotic applications such as object manipulation, autonomous driving, and industrial manufacturing. Major



%Much of the everyday human physical environment is made up of coherent physical objects. Environmental dynamics are well described in terms of the effects of actions on those objects. Perceptual systems are able to report detections of objects with type, location, color, and other properties. Humans naturally designate both goals and prior informa- tion in terms of objects. Thus, it is appropriate for robots to construct ‘‘mental models’’ of their environment that are structured around objects, their properties, and their rela- tions to one another

%To achieve robust, autonomous operation in unstructured
% environments, robots must be able to identify relevant objects and features in their surroundings, recognize the context of the situation, and plan their motions and interactions accord- ingly.



%For robots to effectively operate and interact with objects, they need to understand not only the metric geometry of their surroundings but also its semantic aspects. When requested to organize a room or search for an object, robots must be
%able to reason about object locations and plan goal-directed
%mobile manipulation accordingly. We aim to enable robots
%to semantically map the world at the object level, where the
%representation of the world is a belief over object classes and




==> GeoFusion 3/method.tex <==
%\section{Methodology} \label{sec:method}
%\subsection{Clustering Based Data Association}
%\input{association}
%\subsection{Graph Optimization}
%\input{optimization}
%\subsection{Object Geometric Relationship Inference For Optimization}
%\input{geometry_constraints}



==> GeoFusion 3/optimization.tex <==
\section{Graph Optimization} \label{sec:optimization}
\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{images/factor_graph.jpg}
    \caption{\footnotesize Factor graphs for our two stage optimization method.}
    \label{factor graph}
\end{figure}

% Transition from Data Association
% Two-stage optimization: Stage I and Stage II
% Factor graph definition
% Stage I optimization: Decompose Eq. 3 to two factors
% 1) Odometry measurement factor
% 2) Object measurement factor

After the associations $\mathcal{D}$ between objects $\mathcal{O}$ and semantic measurements $\mathcal{Z}$ have been determined, the most likely robot and object poses are then inferred in the graph optimization process. The factor graph is used to model robot and object states and expresses the conditional independence between them. It gained a huge success in solving SLAM problems \cite{dellaert2017factor} due existing computational tools that allow efficient optimization \cite{dellaert2012factor}. In a factor graph, there exists a set of vertices $\mathcal{V}$ that represent optimization random variables and edges represent factors $\mathcal{F}$ among a subset of random variables. A factor $f$ represents probabilistic dependencies among the random variables and is associated with a cost function. Graphically, the vertex is a circle and the factor is a square in the factor graph, as shown in Fig. \ref{factor graph}. The joint probability of the optimization random variables can be expressed as the product of factors: 

\begin{equation}
    p(\mathcal{V}) \propto \prod_{f \in \mathcal{F}} f(\mathcal{V})
\end{equation}

The optimization process in \GeoFusion is decomposed into two stages, as shown in Fig. \ref{factor graph}. First, 6D pose of the robot and the objects are optimized over odometry and semantic measurements. In the second stage, 6D pose of objects are then fine-tuned over the computed geometric relations to produce a geometric consistent scene estimate.

\subsection{Stage I Optimization}
The right hand side of Eq. \ref{eq:optimization-stage1} is rewritten as:

\begin{equation}
     \log p(\mathcal{Z} | \mathcal{X}, \mathcal{O},  \hat{\mathcal{D}}) 
     = \sum_{t = 1}^T \phi (T_t^{t-1} ; x_{t - 1}, x_t)  + \sum_{t = 1}^T \sum_{k = 1}^{N^t} \phi (z_t^{k, p} ; x_t, o_{d_t^k}^p) \label{eq:optimization-stage1-log} \nonumber
\end{equation}
where $\phi (T_t^{t-1} ; x_{t - 1}, x_t)$ is the odometry factor and $\phi (z_t^{k, p} ; x_t, o_{d_t^k}^p)$ is the object measurement factor. $T_t^{t-1}$ is the odometry measurement between robot pose $x_{t-1}$ and $x_{t}$. $z_t^{k,p}$ is the semantic measurement of an object between the robot pose $x_t$ and the object pose $o_{d_t^k}^p$. With the standard assumption of additive Gaussian noise, each factor follows a quadratic form:

\begin{align}
    \phi (T_t^{t-1} ; x_{t - 1}, x_t) &= - \frac{1}{2} (x_t \ominus x_{t-1} - T_t^{t-1}) Q^{-1} (x_t \ominus x_{t-1} - T_t^{t-1}) \nonumber \\
    \phi (z_t^{k, p} ; x_t, o_{d_t^k}^p) &= - \frac{1}{2} (x_t \ominus o_{d_t^k}^p - z_t^{k, p}) R^{-1} (x_t \ominus o_{d_t^k}^p - z_t^{k, p}) \nonumber
\end{align}
where $ \ominus $ represents the operator that computes the relative transformation. $Q$ and $R$ is the corresponding covariance noise matrix. Thus, The maximum likelihood estimation of $X$ and $O$ can be written as the nonlinear least-squares problem:

\begin{align}
    {\hat{\mathcal{X}}}, {\hat{\mathcal{O}}}^{'} &= 
     \argmin_{\mathcal{X}, \mathcal{O}} \sum_{t=1}^T \| x_{t-1} \ominus x_t - T_{t}^{t-1} \|_{\Sigma_Q} \nonumber \\
     &\quad + \sum_{t=1}^T \sum_{k-1}^{N_t} \| x_t \ominus o_{d_t^k}^p - z_t^{k, p} \|_{\Sigma_R} \footnotemark \label{eq:stage1-least-square} 
\end{align} \footnotetext{$\| X \|_{\Omega} = \sqrt{X^T \Omega X} $}
where $\Sigma_Q$ and $\Sigma_R$ is the information matrix. Note that the as the metrics for translations and rotations are different, the information matrix for them is also different. We use $\Sigma_{p}$ for translations and $\Sigma_{q}$ for rotations which represent as quaternions. $\Sigma_p$ and $\Sigma_{q}$ are diagonal matrices and represent as $Diag(\omega_p, \omega_p, \omega_p)$ and $Diag(\omega_q, 0, 0, 0)$. For symmetric objects in the object measurement factor, we design a separate $Sigma_{q}$ for the rotation. For example, object with rotation axis in z-axis is associated with $\Sigma_q = Diag(0, \omega_q,\omega_q, 0) $ to exclude the influence from z-axis. 


%As shown in Figure \ref{factor graph}, our optimization process is decomposed into two stages. First, 6D pose of the robot and the objects are optimized over odometry and measurements. In the second stage, 6D pose of objects are then fine-tuned over the inferred geometric constraint to generate a geometric consistent scene estimate. To simplify the notation, 6D pose is represented in two ways: a $4 \times 4$ transformation matrix $T$ or a combination of quaternion $q = (r_w, r_x, r_y, r_z)$ and translation $p=(t_x, t_y, t_z)$. Denote $F: T \rightarrow (p,q) $ as the mapping from transformation matrix $T$ to its corresponding quaternion representation $(p, q)$.

% \subsection{Stage I Optimization}

% \subsubsection{Odometry Cost}
%  Odometry measurements provided by ORB-SLAM2 \cite{murAcceptedTRO2015} are used as our initial odometry measurements. The odometry cost describes the difference between the estimated odometry and measured odometry. \newtext{talk about motivation of using odometry estimated from ORB-SLAM2 rather than the raw odometry from wheel encoders}
 
 
% Given the estimated robot poses $x_{t-1},\ x_t$, and the measured odometry $T^t_{t-1}$, we aim to optimize over robot poses $x_t$ and $x_{t-1}$ to minimize the following odometry cost.%  \sui{$T$ is used as different meanings: 6D transformations and odometry cost} 
% \begin{equation}
% \begin{array}{rl}
%     T_{t}^{t-1} &= T_{t-1}^{-1}T_{t} \\ % \text{\sui{do we need this equation?}}\\
%     (p_{t}^{t-1}, q_{t}^{t-1}) &= F(T_{t}^{t-1})\\
%     E_{od} &= ||p_{t}^{t-1}||_{\Sigma_p} + ||q_{t}^{t-1}||_{\Sigma_q}
% \end{array}
% \end{equation}
% where $||p_{t}^{t-1}||_{\Sigma_p}$ is a \textit{diagonally weighted norm} and is computed as $\sqrt{(p_{t}^{t-1})^T \Sigma_p (p_{t}^{t-1}) }$. $\Sigma_p$ is a diagonal matrix and represented as $Diag(\omega_p, \omega_p, \omega_p)$, and $\omega_p$ is the weight of odometry translation. $\Sigma_q = Diag(\omega_q, 0, 0, 0)$, and $\omega_q$ is the weight of odometry rotation. The following appearances of $\omega$ denote the weight of each individual equation unless explicitly explained. %(can be simplified)

% \subsubsection{Measurement Cost}
% Measurement cost \newtext{constrains} the discrepancy between object measurements and estimated object states. %As we have mentioned before, neural network measurements exist many false-positive measurements, and some measurements for symmetric objects are sometimes hard to filter. To reduce the influence of those false measurements in symmetric objects, we design two cost functions for symmetric objects and asymmetric objects separately.
% As mentioned before, neural networks often produce more false positives for symmetric objects due to their symmetries, we design separate cost functions for symmetric and asymmetric objects. 

% Given robot pose $x_t$, measurement $z_t^k$ for object $o_k$, we can get an estimation $\hat{o}_{k, t}$ for $o_k$ at time step t. We aim to optimize over $x_t$ and $o_k$ to minimize the difference between $o_k$ and $\hat{o}_{k, t}$. The relative transform between measurements and optimization is defined as follows:

% \begin{equation}
% \begin{array}{rl}
% T_{\hat{o}_{k, t}} & = T_{x_t}T_{z_t^k} \\%\text{\sui{same here}}\\
% T^{o_{k}}_{\hat{o}_{k, t}} &= T_{o_{k}}^{-1}T_{\hat{o}_{k,t}}\\
% (p^{o_k}_{\hat{o}_{k, t}}, q^{o_k}_{\hat{o}_{k, t}}) &= F(T^{o_k}_{\hat{o}_{k, t}})\\
% \end{array}
% \end{equation}
% For asymmetric object, the cost function is as follows:
% \begin{equation}
%     E_{m} = ||p^{o_k}_{\hat{o}_{k, t}}||_{\Sigma_p} + ||q^{o_k}_{\hat{o}_{k, t}}||_{\Sigma_q}
% \end{equation}
% Here $\Sigma_p = Diag(\omega_p, \omega_p, \omega_p)$, and $\Sigma_q = Diag(\omega_q,0, 0, 0)$.

% As for symmetric object with rotation axis in $z-axis$, the cost function is as follows:
% \begin{equation}
%   E_{m} =||p^{o_k}_{\hat{o}_{k, t}}||_{\Sigma_p} + ||q^{o_k}_{\hat{o}_{k, t}}||_{\Sigma_q}
% \end{equation}
% where $ \Sigma_p = Diag(\omega_p, \omega_p, \omega_p)$ and $\Sigma_q = Diag(0, \omega_q,\omega_q, 0) $. The last term of $\Sigma_q$ is set to zero to exclude the influence from the z-axis. For those objects whose rotation axis is in other axis, the cost functions can be derived in the similar way.

\input{geometry_constraints}

==> GeoFusion 3/relatedwork.tex <==
\section{related work}
%Our work builds a semantic map at the object-level given noisy semantic measurements. Geometric consistency is exploited for robust data association and is modeled in the graph optimization for better scene understanding. 
%We discuss related work in a) semantic mapping and b) scene estimation. 

% additional work to be cited
% Semantic Structure From Motion with Points, Regions, and Objects
% Context-Coherent Scenes of Objects for Camera Pose Estimation
% Detect-SLAM: Making Object Detection and SLAM Mutually Beneficial
% An Orientation Factor for Object-Oriented SLAM

\subsection{Semantic Mapping}
From the emerging of semantic mapping \cite{kuipers2000spatial}, lots of work have explored this field with various semantic representations \cite{kostavelis2015semantic}. With the focus on the object-level semantic map, one widely used approach is to reconstruct a 3D map from either sparse features \cite{murAcceptedTRO2015} or dense point clouds \cite{newcombe2011kinectfusion, whelan2015elasticfusion, Rosinol20icra-Kimera} and then augments the map with the objects. Civera et al. \cite{civera2011towards} and Ekvall et al. \cite{ekvall2006integrating} used SURF/SIFT descriptors to register objects to the map created in a parallel thread. However, their work can not deal with objects in clutter. To deal with clutter, Li et al. \cite{li2016incremental} proposed an incremental segmentation approach to fuse segmentation across different frames based on dense reconstruction 3D map and used ObjRecRANSAC \cite{papazov2010efficient} to register object poses. But their method does not scale well with substantial false detections. 

Salas-Moreno et al. \cite{salas2013slam++} proposed an object SLAM system that recognized objects using Point-Pair Features in each frame and directly performed graph optimization on object and camera 6D poses. Their work shows promising results in the direction of building maps with 6D object poses. McCormac et al. \cite{mccormac2018fusion++} constructed an online object-level SLAM system with previously unknown shape and perform pose graph optimization at the object level. Both of their work assume independence between objects and hence difficult to work well in densely cluttered environments. Zeng et al. \cite{zeng2018semantic} proposed CT-MAP, which considers contextual relation between objects and temporal consistency of object poses in a conditional random field and maintain belief over object classes and poses. This approach is robust to false detections; however, does not scale well to the increasing number of objects due to the nature of pure generative inference. 

%fuses 3D point cloud to produce a dense reconstruction \cite{newcombe2011kinectfusion, whelan2015elasticfusion} and then augment the map with objects using segmentation and registration \cite{tateno20162, li2016incremental}. 



%ne solution to this problem is to perform 3D dense reconstruction \cite{newcombe2011kinectfusion, whelan2015elasticfusion} which fuses 3D point clouds at the geometric level from consecutive views first, and then segment and identify objects from the fused point cloud \cite{tateno20162, li2016incremental}. These methods work well in large scale environments however becomes fragile when the scene becomes densely cluttered where multiple objects are placed in close contact or there are substantial false positive observations. Another way is to directly perform fusion on higher level semantics like object identities and 6D poses and optimize over object pose graph \cite{salas2013slam++, mccormac2018fusion++}. We more interested in this direction since an awareness of object instance as the observations can provide more meaningful information when facing more cluttered scenes as shown in Fix xx. 


% object-level semantic mapping \\
% three categories: \\
% 1. fusion point cloud and perform segmantation \\
% 2. filtering based approach \\
% 3. graph optimziation on object-level \\

\subsection{Scene Estimation}
Great progress has been made by deep neural networks in object detection \cite{ren2015faster, he2017mask}, 6D object pose estimation \cite{xiang2017posecnn, wang2019densefusion} and semantic segmentation \cite{long2015fully}. To be robust to false detections due to the effects of overfitting, discriminative-generative algorithms \cite{narayanan2016discriminatively, sui2017sum} have been proposed for robust perception, especially in adversarial environments \cite{chen2019grip}. These efforts combine inference by deep neural networks  with sampling and probabilistic inference models to achieve robust and adaptive perception. However, the robustness is at the cost of computation time and the assumption object independence. 

Sui et al. \cite{sui2017goal} propose an axiomatic scene estimation method to estimate both geometric spatial relationships between objects and their 3D object poses for goal-directed manipulation. The spatial relation introduces strong constraints to reduce the search space of object poses. Desingh et al. \cite{desingh2016physically} and Mitash et al. \cite{mitash2019physics} leverage physics into scene estimation to search object poses based on compatibility score from physics simulation. The above-mentioned methods take either geometric and physical constraints into account for searching object poses, at the cost of computational efficiency.
%however not very efficient. 


%\subsection{Scene Estimation with Geometric Relations}

% ctmap

% skipmap++ 
% http://openaccess.thecvf.com/content_ICCV_2017_workshops/papers/w13/De_Gregorio_SkiMap_Real-Time_Mapping_ICCV_2017_paper.pdf


% Incremental scene understanding on dense SLAM


% slam++

% Semantic Structure from Motion

%mccormac2018fusion++ reconstructs object meshes online and track them in SLAM framework
%maskfusion uses elastic fusion and tracks dynamic objects



%A goal-directed task planner with a state space formalization becomes a common component for robot applications. Facing an incomplete state space, uncertainty and faults, a state space can be highly complex and difficult to scale \cite{chen2016planning}. A classical method to plan in a complex environment with incomplete information is planning with sensing actions \cite{Puigbo_article}. This method is able to generate a short term plan quickly. But without consideration of missing information and uncertainty, the plan is not robust and efficient in long term consideration. \cite{dearden2013approach} use completely symbolic planning on manipulation and generate a geometric plan by translating the symbolic predicates into geometric relationships. When one execution fails, the method backtracks first in geometric level, then in symbolic level.



%Other approaches are planning under belief space, which integrate planning of perception and action by modelling the state space with probability distributions. Some related works try to reduce the scale of the belief state in real world problem by ignoring marginal parts in belief space \cite{feng2005efficient} or compress random variables \cite{poupart2003value}. However, the fundamental issue of large scaling remains. As the task grows more complex, a long time plan becomes intractable. 
% Recent research [12], [13], [14] has established the value of control in belief space using simplified models and replanning. 

%One way to model goal-directed manipulation tasks with uncertainty treats this task as a partially observable Markov decision process (POMDP) problem.  With a proper but extremely complex description of environment \cite{Papadimitriou:1987:CMD:35577.35581}, a POMDP solver is enough to generate a variety of real-world sequential decision processes. State-of-the-art POMDP methods are able to yield good policies for problems with thousands of states with constrains \cite{Smith2005542}\cite{silver2010monte}. Several approaches are used to represent probability distributions in a more efficient way, such as using particle filtering to describe probability distributions \cite{PAJARINEN2017213}, in order to make POMDPs tractable with large state spaces. Another method to approximate the complex state space is using most likelihood assumption such as Q-MDP \cite{Littman95}. This approach considers uncertainty in the current process dynamics, but assumes no state uncertainty exists in the future. Under the fundamental limitation of computational ability and modeling real world, approximations and simplifications are inevitable in POMDP problems. \cite{pajarinen2017robotic} proposed an online POMDP for robot manipulation in a cluttered environment, but this method only looking forward a very short-term action series which makes it difficult to deployed to a task requires long time horizons.

%\cite{kaelbling2012unifying} integrated the perception, estimation, and action in the belief space for complex robot grasping task. The method is able to tackle the environment uncertainty by model the state into probability distribution. Our method shares similar idea however our method takes false detections into account and works with the complex task. 







==> implementation.tex <==
\section{implementation}
\subsection{Object Detection and Pose Estimation}

For particle filtering, we employ the CUDA-OpenGL
interoperation to render all particles in a single render buffer
on the GPU and can be accessed by the CUDA kernels to
compute the weights for particles. The major computation
is operated on directly on GPU and there is very few data
transfer between GPU and CPU memory. It provides a
tractable solution for us to employ more particles to sample
hypothesized objects
\subsection{Grasp and Place}
Graspable poses for each objects are generated based on geometry models or using grasp points generator(GPG) in local frame. A point cloud based collision checker is implemented. All collision free graspable poses are kept and ranked. Graspable poses whose grasp points are closer to the center of target objects and whose axes through both finger tips are more parallel to the surface of table (to avoid poses where one finger is under objects) are given higher priority. 

Objects are placed according to a placing policy. In the placement algorithm, all the objects are represented by cuboids, and will be placed firmly on a plane. We use RANSAC to segment horizontal planes from the point cloud of the box and search among the planes to find a rectangle area with enough support for objects (either the center of the objects should be projected in the polygon surrounded by the support points or more than 70\% area around the center are supported). Place poses are ranked according the closeness to the ideal placement height given by the planner. Among the place poses with similar height, a better place position for regular object is close to the back center of the box; for vertical objects, a better pose is close to the two sides of the box. After checking the collision between the poses of objects and gripper with box point cloud, the place poses are given to MoveIt! to perform motion planning afterwards.

==> method.tex <==
%\section{Methodology} \label{sec:method}
%\subsection{Clustering Based Data Association}
%\input{association}
%\subsection{Graph Optimization}
%\input{optimization}
%\subsection{Object Geometric Relationship Inference For Optimization}
%\input{geometry_constraints}


